Fairness-Accuracy Trade-Offs: A Causal Perspective

Systems based on machine learning may exhibit discriminatory behavior based on sensitive characteristics such as gender, sex, religion, or race. In light of this, various notions of fairness and methods to quantify discrimination were proposed, leading to the development of numerous approaches for constructing fair predictors. At the same time, imposing fairness constraints may decrease the utility of the decision-maker, highlighting a tension between fairness and utility. This tension is also recognized in legal frameworks, for instance in the disparate impact doctrine of Title VII of the Civil Rights Act of 1964 -- in which specific attention is given to considerations of business necessity -- possibly allowing the usage of proxy variables associated with the sensitive attribute in case a high-enough utility cannot be achieved without them. In this work, we analyze the tension between fairness and accuracy from a causal lens for the first time. We introduce the notion of a path-specific excess loss (PSEL) that captures how much the predictor's loss increases when a causal fairness constraint is enforced. We then show that the total excess loss (TEL), defined as the difference between the loss of predictor fair along all causal pathways vs. an unconstrained predictor, can be decomposed into a sum of more local PSELs. At the same time, enforcing a causal constraint often reduces the disparity between demographic groups. Thus, we introduce a quantity that summarizes the fairness-utility trade-off, called the causal fairness/utility ratio, defined as the ratio of the reduction in discrimination vs. the excess loss from constraining a causal pathway. This quantity is suitable for comparing the fairness-utility trade-off across causal pathways. Finally, as our approach requires causally-constrained fair predictors, we introduce a new neural approach for causally-constrained fair learning.

==> sections/C1Checklist.tex <==
\section*{Reproducibility Checklist}

Unless specified otherwise, please answer “yes” to each question if the relevant information is described either in the paper itself or in a technical appendix with an explicit reference from the main paper. If you wish to explain an answer further, please do so in a section titled “Reproducibility Checklist” at the end of the technical appendix.

This paper:

\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced \textbf{yes}
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results \textbf{yes}
    \item Provides well marked pedagogical references for less-familiar readers to gain background necessary to replicate the paper \textbf{yes}
\end{itemize}

Does this paper make theoretical contributions? \textbf{yes}

If yes, please complete the list below.

\begin{itemize}
    \item All assumptions and restrictions are stated clearly and formally. \textbf{yes}
    \item All novel claims are stated formally (e.g., in theorem statements). \textbf{yes}
    \item Proofs of all novel claims are included. \textbf{yes, Appendix~\ref{appendix:theorem-proofs}}
    \item Proof sketches or intuitions are given for complex and/or novel results. \textbf{yes, Appendix~\ref{appendix:theorem-proofs}}
    \item Appropriate citations to theoretical tools used are given. \textbf{yes}
    \item All theoretical claims are demonstrated empirically to hold. \textbf{yes}
    \item All experimental code used to eliminate or disprove claims is included. \textbf{yes}
\end{itemize}

Does this paper rely on one or more datasets? \textbf{yes}

If yes, please complete the list below.

\begin{itemize}
    \item A motivation is given for why the experiments are conducted on the selected datasets \textbf{yes, Section~\ref{sec:experiments}, Appendix~\ref{appendix:experiments}}
    \item All novel datasets introduced in this paper are included in a data appendix. \textbf{NA, using known datasets}
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \textbf{NA, using known datasets}
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. \textbf{yes}
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. \textbf{yes}
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisfying. \textbf{NA, datasets are public}
\end{itemize}

Does this paper include computational experiments? \textbf{yes}

If yes, please complete the list below.

\begin{itemize}
    \item Any code required for pre-processing data is included in the appendix. \textbf{yes, together with an anonymized repository}
    \item All source code required for conducting and analyzing the experiments is included in a code appendix. \textbf{yes}
    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \textbf{yes}
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from \textbf{yes}
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. \textbf{yes, seed is set at the beginning of each script}
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. \textbf{yes, in the Appendix}
    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. \textbf{yes, Section~\ref{sec:experiments}, Appendix~\ref{appendix:experiments}}
    \item This paper states the number of algorithm runs used to compute each reported result. \textbf{yes}
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. \textbf{yes}
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). \textbf{yes}
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. \textbf{yes}
    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. \textbf{yes}
\end{itemize}

